Potential Applications of Quantum Computing at Los Alamos National Laboratory

The emergence of quantum computing technology over the last decade indicates the potential for a transformational impact in the study of quantum mechanical systems. It is natural to presume that such computing technologies would be valuable to large scientific institutions, such as United States national laboratories. However, detailed descriptions of what these institutions would like to use these computers for are limited. To help provide some initial insights into this topic, this report develops detailed use cases of how quantum computing technology could be utilized to enhance a variety of quantum physics research activities at Los Alamos National Laboratory, including quantum magnetic materials, high-temperature superconductivity and nuclear astrophysics simulations. The report discusses how current high-performance computers are used for scientific discovery today and develops detailed descriptions of the types of quantum physics simulations that Los Alamos National Laboratory scientists would like to conduct, if a sufficient computing technology became available. While the report strives to highlight the breadth of potential application areas for quantum computation, this investigation has also indicated that many more use cases exist at Los Alamos National Laboratory, which could be documented in similar detail with sufficient time and effort.

==> commands.tex <==
%create command for markings on top and bottom of page
%change font size/color/etc here to maintain consistency
\newcommand\topMarkings[1]{%
\renewcommand\@topMarkings{\markingfont#1}%
}
\newcommand\@topMarkings{}

\newcommand\bottomMarkings[1]{%
\renewcommand\@bottomMarkings{\markingfont#1}%
}
\newcommand\@bottomMarkings{}

\newcommand\markings[1]{%
\topMarkings{\markingfont#1}
\bottomMarkings{\markingfont#1}
%\renewcommand\@markings{\markingfont#1}%
}
\newcommand\@markings{}


%redefine \section to save section title for putting in header and resets page number to 1
\newcommand\appendixmode[1]{%
\renewcommand\@appendixmode{#1}%
}
\newcommand\@appendixmode{}

\newcommand\appendixSections[1]{%
\if\relax\noexpand#1\relax
\appendixmode{}
\else 
\appendixmode{1}
\fi
}

\newcommand\sectiontitle{}
\newcommand\subsectiontitle{}
\newcommand\subsubsectiontitle{}
\let\oldsection\section
\let\oldsubsection\subsection
\let\oldsubsubsection\subsubsection
\let\oldpage\thepage

\newcounter{@secnumdepth}

\usepackage{titletoc}

\RenewDocumentCommand{\section}{s o m}{%
\FloatBarrier  
    \setcounter{figure}{0}\setcounter{table}{0}%\setcounter{tocdepth}{0}
  \IfBooleanTF{#1}
    {\setcounter{@secnumdepth}{\value{secnumdepth}}% Store secnumdepth
     \setcounter{secnumdepth}{0}% Print only up to \chapter numbers
     \clearpage{\thispagestyle{markings}\cleardoublepage}\setcounter{page}{1}\oldsection{#3}\renewcommand{\sectiontitle}{#3}% \section*
     \setcounter{secnumdepth}{\value{@secnumdepth}} }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\clearpage{\thispagestyle{markings}\cleardoublepage}\setcounter{page}{1}\oldsection[#2]{#3}\renewcommand{\sectiontitle}{#3}}% \section[.]{..}
       {\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{contents}}\setcounter{page}{1}\oldsection{#3}\renewcommand{\sectiontitle}{#3}}}%
       \pagestyle{contents}% \section{..}
 \renewcommand{\thepage}{\thesection-\arabic{page}}\renewcommand\thefigure{\thesection-\arabic{figure}}\renewcommand\thetable{\thesection-\arabic{table}} \label{#3}%
\FloatBarrier%

       %\addtocontents{toc}{\contentsline{section}{\numberline{\thesection}\sectiontitle}{\thesection-\thepage}}

}

\RenewDocumentCommand{\subsection}{s o m}{%
\FloatBarrier 
\IfBooleanTF{#1}
{\oldsubsection*{#3}}
{\IfValueTF{#2}% \section
    {\oldsubsection[#2]{#3}}
    {\oldsubsection{#3}}
    }
\FloatBarrier
}%

\RenewDocumentCommand{\subsubsection}{s o m}{%
\FloatBarrier 
\IfBooleanTF{#1}
{\oldsubsubsection*{#3}}
{\IfValueTF{#2}% \section
    {\oldsubsubsection[#2]{#3}}
    {\oldsubsubsection{#3}}
    }
\FloatBarrier
}%




%create new variable to store start page number for executive summary
%used to prevent section title from being in header on first page
%avoid using \renewcommand, as \executivepage will update with \thepage, rather than keeping its original value


\NewDocumentCommand{\frontmattersection}{s o m}{%
\FloatBarrier\setcounter{figure}{0}\setcounter{table}{0}%
  \IfBooleanTF{#1}
    {\setcounter{@secnumdepth}{\value{secnumdepth}}% Store secnumdepth
     \setcounter{secnumdepth}{0}% Print only up to \chapter numbers
     \clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{frontmatter}}\oldsection{#3}\renewcommand{\sectiontitle}{#3}% \section*
     \setcounter{secnumdepth}{\value{@secnumdepth}} }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{frontmatter}}\oldsection[#2]{#3}\renewcommand{\sectiontitle}{#3}}% \section[.]{..}
       {\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{frontmatter}}\oldsection{#3}\renewcommand{\sectiontitle}{#3}}}%
       \pagestyle{frontmatter}% 
       \renewcommand{\thepage}{\roman{page}}%
       \edef\startPage{\thepage}%\section{..}%
        \label{#3}\FloatBarrier%
        
}






\newcounter{@appendixnumber}
\setcounter{@appendixnumber}{0}
\NewDocumentCommand{\appendixsection}{s o m}{%
\FloatBarrier
  \setcounter{figure}{0}
  \setcounter{table}{0}
   \setcounter{subsection}{0}


     \clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{appendix}}\stepcounter{@appendixnumber}\setcounter{page}{1}\renewcommand{\sectiontitle}{Appendix\hspace{2pt}\Alph{@appendixnumber}:\hspace{4pt}#3}\titleformat{\section}{\heading\selectfont}{}{0pt}{}[]\renewcommand{\thesection}{\Alph{@appendixnumber}}\phantomsection\oldsection*{\sectiontitle}%% \section*
    \stepcounter{section}
    \pagestyle{appendix}% \section{..}
       
    \renewcommand{\thepage}{\Alph{@appendixnumber}-\arabic{page}}\renewcommand\thefigure{\Alph{@appendixnumber}-\arabic{figure}}\renewcommand\thetable{\Alph{@appendixnumber}-\arabic{table}}\label{#3}\FloatBarrier%
    
    %add TOC entry.  Allow TOC name to be passed with [] option when section is created
    \IfValueTF{#2}%
    {\addcontentsline{toc}{section}{Appendix\hspace{2pt}\Alph{@appendixnumber}:\hspace{4pt}#2}}
    {\addcontentsline{toc}{section}{\sectiontitle}}
}%
  


\NewDocumentCommand{\appendixsubsection}{s o m}{%
\FloatBarrier
\setcounter{subsubsection}{0}
  \IfBooleanTF{#1}
    {
     \renewcommand{\subsectiontitle}{#3}\oldsubsection{#3}% \section*
      }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\renewcommand{\subsectiontitle}{#3}}\oldsubsection[#2]{\subsectiontitle}% \section[.]{..}
       {\oldsubsection{#3}\renewcommand{\subsectiontitle}{#3}}}%
       \titleformat{\subsection}{\subheading\selectfont}{}{0pt}{}[]%
    \FloatBarrier
}%

\NewDocumentCommand{\appendixsubsubsection}{s o m}{%

\FloatBarrier
  \IfBooleanTF{#1}
    {
     \renewcommand{\subsubsectiontitle}{#3}\oldsubsubsection{#3}% \section*
      }% Restore secnumdepth
    {\IfValueTF{#2}% \section
       {\renewcommand{\subsubsectiontitle}{#3}}\oldsubsubsection[#2]{\subsubsectiontitle}% \section[.]{..}
       {\oldsubsubsection{#3}\renewcommand{\subsubsectiontitle}{#3}}}%
       \titleformat{\subsubsection}{\subsubheading\selectfont}{}{0pt}{}[]%
     \FloatBarrier
}%



\let\oldprintbibliography\printbibliography%
\newcommand{\ShowBibliography}[0]{%
\clearpage{\thispagestyle{markings}\cleardoublepage\thispagestyle{contents}}%

\thispagestyle{contents}%
\setcounter{@appendixnumber}{18}%
\renewcommand{\sectiontitle}{References}%
\renewcommand{\thepage}{R-\oldpage}%
%print heading then change page style contents, then print biblio without heading
%needed otherwise first page will have wrong page style
\printbibheading
\thispagestyle{contents}
\pagestyle{contents}
\oldprintbibliography[heading=none]


\renewcommand{\thepage}{R-\oldpage}%
}%

\begin{comment}
\RenewDocumentCommand{\printbibliography}{s o m}{%
%{\clearpage{\thispagestyle{markings}\cleardoublepage}%
%}%
%\thispagestyle{contents}
%\setcounter{@appendixnumber}{18}
%\renewcommand{\sectiontitle}{References}
\oldprintbibliography
%\thispagestyle{contents}
%
%\renewcommand{\thepage}{R-\oldpage}%
}%




\let\oldprintbibliography\printbibliography
\RenewDocumentCommand{\printbibliography}{s o m}{%
\oldprintbibliography%
\renewcommand{\sectiontitle}{References}
%\thispagestyle{references}%
\renewcommand{\thepage}{R-\oldpage}%
}
\end{comment}

%Redefine TOC so page doesn't reset and it keeps the right pagestyle
\let\oldtableofcontents\tableofcontents
\renewcommand{\tableofcontents}{%
   \pagestyle{markings} \cleardoublepage \pagestyle{contents}
   \edef\startPage{\thepage}
   
\tocloftpagestyle{contents}
\renewcommand{\sectiontitle}{Contents}
\let\oldoldsection\section
\renewcommand{\section}{\oldsection}
\renewcommand{\thepage}{\roman{page}}
\renewcommand{\cftsecleader}{\cftdotfill{\cftdotsep}}


%make a TOC
\oldtableofcontents

%set so up to subsubsections are shown in TOC
\setcounter{tocdepth}{3}

%disable \clearpage so list of figure and tables don't create a new page and are listed directly after TOC
\let\LaTeXStandardClearpage\clearpage
\let\clearpage\relax
  % Do nothing when a \clearpage command appears 
\renewcommand{\listfigurename}{Figures}
\listoffigures
\pagestyle{frontmatter}
\renewcommand{\listtablename}{Tables}
\listoftables
\let\clearpage\LaTeXStandardClearpage % Return to the old definition


%reset section definition 
\let\section\oldoldsection

\let\chapter\section
\let\section\subsection
\let\subsection\subsubsection
\let\subsubsection\paragraph
\let\paragraph\subparagraph
}



==> fonts.tex <==
%%%%%%%%%%Set Caption Font%%%%%%%%%
\usepackage{caption}
\DeclareCaptionFont{caption}{\sourcesanspro\captiongrey\fontsize{9}{12}\selectfont}
\usepackage[font=caption]{caption}



%%%%%%%%%%%LANL colors%%%%%%%%%%%%%
\newcommand{\primarycolor}{\color[HTML]{000F7E}}
\newcommand{\primarygradient}{\color[HTML]{090238}}
\newcommand{\secondarycolor}{\color[HTML]{0070C1}}
\newcommand{\secondarycolortwo}{\color[HTML]{3296DC}}
\newcommand{\secondarycolorthree}{\color[HTML]{69C3FF}}
\newcommand{\captiongrey}{\color[HTML]{555962}}


%%%%%%%%%%%%Fonts%%%%%%%%%%%%%%%%%%%%
%fonts from style guide note: acumin not avaialable in latex, using URW Grotesk
%acumin used for heading, source sans pro used for body, captions, etc.
\newcommand{\acumin}{\fontfamily{ugq}}
\newcommand{\sourcesanspro}{\fontfamily{SourceSansPro-TLF}}

%font types listed in style guide
\newcommand{\fontone}{\acumin \fontsize{38}{40}\fontseries{bx}}
\newcommand{\fonttwo}{\acumin \fontsize{24}{28}\fontseries{b}}
\newcommand{\fontthree}{\sourcesanspro \fontsize{15}{22}\fontseries{b}}
\newcommand{\fontfour}{\sourcesanspro \fontsize{10}{14}\fontseries{sb}}
\newcommand{\fontfive}{\sourcesanspro \fontsize{10}{14}}

%define fonts for headings in Word report template
\newcommand{\headingfont}{\acumin \fontsize{14}{18}\fontseries{bx}}
\newcommand{\subheadingfont}{\acumin \fontsize{12}{16}\fontseries{b}}
\newcommand{\subsubheadingfont}{\acumin \fontsize{11}{15}\fontshape{it}}

%define fonts+color for use in headings
\newcommand{\heading}{\headingfont\primarycolor}
\newcommand{\subheading}{\subheadingfont\primarycolor}
\newcommand{\subsubheading}{\subsubheadingfont\primarycolor}


\newcommand{\tableheading}{\acumin\fontseries{bx}\fontsize{11}{12}\selectfont}
\newcommand{\markingfont}{\sourcesanspro\fontsize{14}{0}\fontseries{bx}\selectfont}
\newcommand{\OUOfont}{\markingfont}
\newcommand{\ClassfiedFont}{\color{red}\markingfont}

\newcommand{\SRD}{\color{red}\markingfont SECRET//RESTRICTED DATA}
\newcommand{\OUO}{\OUOfont Official Use Only}
%\newcommand{\markingfont}{\acumin\color{red}\fontsize{20}{0}\fontseries{bx}\selectfont}
%\newcommand{\captionfont}{\sourcesanspro\fontsize{9}{12}\selectfont}
%define section headers as shown in word template



%add [runin] after {\section} if you don't want new line after header
%{xxpt} controls distance between section number and section title
\titleformat{\section}{\heading\selectfont}{\thesection}{10pt}{}[]
\titleformat{\subsection}{\subheading\selectfont}{\thesubsection}{10pt}{}[]
\titleformat{\subsubsection}{\subsubheading\selectfont}{\thesubsubsection}{10pt}{}[]


==> pagestyles.tex <==
%%%%%%%%%%%%page styles%%%%%%%%%%%
%Generic markings page
\fancypagestyle{markings}{\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[C]{ \vspace{30pt}  \@bottomMarkings } \fancyhead[C]{\@topMarkings } }

%Exectuive Summary page style
\fancypagestyle{frontmatter}{  \fancyhf{}\renewcommand{\headrulewidth}{0pt}

\fancyhead[EL]{\begin{center}\@topMarkings\end{center} \heading\selectfont\sectiontitle }


%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center} \leavevmode \\ 
\ifthenelse{\equal{\thepage}{\startPage}}{}{\heading\selectfont\sectiontitle}
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
        \raggedright Page \quad \thepage \hfill Los Alamos National Laboratory \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }% 
}

\fancypagestyle{}{\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[C]{ \@bottomMarkings } \fancyhead[C]{\@topMarkings}}



%Title page, includes markings and LANL logo in bottom left of footer
\fancypagestyle{title}{\pagenumbering{roman}\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[L]{\hspace*{-0.5in}\begin{tikzpicture}
  \node[opacity=0.5,inner sep=0pt] at (0,0)
   {\includegraphics[scale=.75]{LANL_Logo_Ultramarine.png}};
  \end{tikzpicture} \leavevmode \\ \begin{center}\@bottomMarkings\end{center}} \fancyhead[C]{\@topMarkings}}
  
  
%Preparation page, has LANL logo and disclaimer with markings below 
 \fancypagestyle{preparation}{\fancyhf{}\renewcommand{\headrulewidth}{0pt}\fancyfoot[L]{\begin{tikzpicture}
  \node[opacity=0.5,inner sep=0pt] at (0,0)
   {\includegraphics[scale=.75]{LANL_Logo_Ultramarine.png}};
  \end{tikzpicture} \leavevmode \\ 
\fontsize{8}{10}\selectfont\noindent Los Alamos National Laboratory, an affirmative action/equal opportunity employer, is managed by Triad National Security, LLC, for the National Nuclear Security Administration of the U.S. Department of Energy, under contract 89233218CNA000001. By acceptance of this article, the publisher recognizes that the U.S. Government retains a nonexclusive, royalty-free license to publish or reproduce the published form of this contribution, or to allow others to do so, for U.S. Government purposes. Los Alamos National Laboratory requests that the publisher identify this article as work performed under the auspices of the U.S. Department of Energy. Los Alamos National Laboratory strongly supports academic freedom and a researcher’s right to publish; as an institution, however, the Laboratory does not endorse the viewpoint of a publication or guarantee its technical correctness.
  \leavevmode \\
  \begin{center}\vspace{30pt}\@bottomMarkings\end{center}} 
  
  
  \fancyhead[C]{\@topMarkings}}

%Contents pages, includes centered markings and section header on the left/right for even/odd pages
\fancypagestyle{contents}{%

%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}

\fancyhead[EL]{\begin{center}\@topMarkings\end{center}\heading\selectfont\sectiontitle }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center}  \leavevmode \\ \ifthenelse{\equal{\value{page}}{1}}{}{\heading\selectfont\sectiontitle}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
        \raggedright Page \quad \thepage \hfill Los Alamos National Laboratory \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }%
}


%references pages, includes centered markings and section header on the left/right for even/odd pages
\fancypagestyle{references}{%
%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}

\fancyhead[EL]{\begin{center}\@topMarkings\end{center}\heading\selectfont\sectiontitle }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center}  \leavevmode \\ \ifthenelse{\equal{\value{page}}{1}}{}{\heading\selectfont\sectiontitle}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
        \raggedright Page \quad \thepage \hfill Los Alamos National Laboratory \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }%


}


\fancypagestyle{appendix}{%
%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}


\fancyhead[EL]{\begin{center}\@topMarkings\end{center} \heading\selectfont\sectiontitle }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center} \leavevmode \\ \ifthenelse{\oldpage=1}{}{\heading\selectfont\sectiontitle}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad \thepage \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
        \raggedright Page \quad \thepage \hfill Los Alamos National Laboratory \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }%
}

\fancypagestyle{references}{%
%\pagenumbering{arabic}
\fancyhf{}\renewcommand{\headrulewidth}{0pt}


\fancyhead[EL]{\begin{center}\@topMarkings\end{center} \heading\selectfont References }

%Add section title to right part of header, unless first page of a new section
\fancyhead[OR]{\begin{center}\@topMarkings\end{center} \leavevmode \\ \ifthenelse{\thepage=1}{}{\heading\selectfont References}%
}
    
    
    \fancyfoot[O]{\raggedright \@title \leavevmode \\
        \raggedright Los Alamos National Laboratory \hfill Page\quad R-\thepage \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }
    
    \fancyfoot[E]{\raggedleft \@title \leavevmode \\
        \raggedright Page \quad R-\thepage \hfill Los Alamos National Laboratory \leavevmode \\
        \begin{center}\@bottomMarkings\end{center}
    }%
}


